Pay Transparency and Gender Equality

Since 2018 UK firms with at least 250 employees have been mandated to publicly disclose gender equality indicators. Exploiting variations in this mandate across firm size and time we show that pay transparency closes 18 percent of the gender pay gap by reducing men's wage growth. The public availability of the equality indicators seems to influence employers' response as worse performing firms and industries more exposed to public scrutiny reduce their gender pay gap the most. Employers are also 9 percent more likely to post wages in job vacancies, potentially in an effort to improve gender equality at entry level.

==> Tables/GPG_FAME_selection.tex <==
\begin{table}[htbp]
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{ {Gender equality performance and presence in FAME}}\label{selectivity_gpg_fame}
\scalebox{0.9}{
%\adjustbox{max height=\dimexpr\textheight-5.3cm\relax,
%          max width=\textwidth}{
\begin{threeparttable}
\begin{footnotesize}
\begin{tabular}{l*{8}{c}}
\toprule
                   &\multicolumn{4}{c}{2017/18}&\multicolumn{4}{c}{2018/19}\\
                  \cmidrule(l){2-5} \cmidrule(l){6-9} &\multicolumn{1}{c}{Entire}&\multicolumn{2}{c}{Merged with FAME}&\multicolumn{1}{c}{P-value}&\multicolumn{1}{c}{Entire}&\multicolumn{2}{c}{Merged with FAME}&\multicolumn{1}{c}{P-value}\\
                    &\multicolumn{1}{c}{sample}&\multicolumn{1}{c}{No}&\multicolumn{1}{c}{Yes}&\multicolumn{1}{c}{difference}&\multicolumn{1}{c}{sample}&\multicolumn{1}{c}{No}&\multicolumn{1}{c}{Yes}&\multicolumn{1}{c}{difference}\\
    
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    
\midrule
Gender pay gap & 11.79 & 11.89 & 11.77 & 0.78 & 11.88 & 11.55 & 11.94 & 0.35\\
 & (15.84) & (13.46) & (16.25) &  & (15.51) & (13.40) & (15.86) & \\

\addlinespace
Observations & 10,557 & 1,691 & 8,866 &  & 10,812 & 1,660 & 9,152 & \\
\bottomrule
\end{tabular}
\end{footnotesize}
\begin{tablenotes}
\item{\footnotesize \textit{Source:} GEO 2018--2019, FAME, 2013--2019.}
\item {\footnotesize \textit{Notes:} This table explores potential selection patterns of GEO firms that we merge with FAME. Columns 1 and 5 reports the gender median hourly pay gap for all GEO firms in 2017/2018 and 2018/2019, Column 2 and 6 refer to firms that we do find in FAME, Columns 3 and 7 refer to firms that we merge with FAME, and Columns 4 and 8 report the p-value of the difference in the sample means of these two groups in each year. }
\item{\footnotesize *** p$<$0.01, ** p$<$0.05, * p$<$0.1.}
\end{tablenotes}
\end{threeparttable}}
\end{table}
